PhyCustom: Towards Realistic Physical Customization in Text-to-Image Generation

Recent diffusion-based text-to-image customization methods have achieved significant success in understanding concrete concepts to control generation processes, such as styles and shapes. However, few efforts dive into the realistic yet challenging customization of physical concepts. The core limitation of current methods arises from the absence of explicitly introducing physical knowledge during training. Even when physics-related words appear in the input text prompts, our experiments consistently demonstrate that these methods fail to accurately reflect the corresponding physical properties in the generated results. In this paper, we propose PhyCustom, a fine-tuning framework comprising two novel regularization losses to activate diffusion model to perform physical customization. Specifically, the proposed isometric loss aims at activating diffusion models to learn physical concepts while decouple loss helps to eliminate the mixture learning of independent concepts. Experiments are conducted on a diverse dataset and our benchmark results demonstrate that PhyCustom outperforms previous state-of-the-art and popular methods in terms of physical customization quantitatively and qualitatively.

==> resources/tables/cvpr2025_rebuttal.tex <==
%%%%%%%%%%%%% 2023/07/25 update %%%%%%%%%%%%%

\begin{table}[t]
    \centering
    \begin{adjustbox}{width=\linewidth}
	\begin{threeparttable}
        \begin{tabular}{l|c|ccc|cc}
            \toprule
            Method & Venue & CLIP-V $\uparrow$ & CLIP-V-O $\uparrow$ & LLM $\uparrow$ & \re{Train(s) $\downarrow$} & \re{Infer(s) $\downarrow$} \\
            \midrule
            DreamBooth & CVPR 2023 & 0.265 & 0.293 & 78.7\% & 195.42 & 2.84 \\
            IP-adapter & Arxiv 2023 & 0.236 & 0.311 & 73.6\% & - & 2.28 \\
            Custom Diff & CVPR 2023 & 0.255 & 0.303 & 82.7\% & 243.19 & 2.04 \\
            \re{Blip-diffusion} & NeurIPS 2024 & 0.264 & 0.273 & 78.0\% & - & 2.91 \\
            \re{FreeCustom} & CVPR 2024 & 0.243 & 0.297 & 82.9\% & - & 23.78 \\
            \re{InstantStyle} & Arxiv 2024 & 0.233 & 0.299 & 71.6\% & - & \textbf{1.34} \\
            % \re{DreamMix}~\cite{yang2024dreammix} & Arxiv 2024 \\
            \midrule
            PhyDiff & - & \textbf{0.267} & \textbf{0.319} & \textbf{84.0\%} & \textbf{112.17} & 5.72 \\
            \bottomrule
        \end{tabular}
        \end{threeparttable}
    \end{adjustbox}
    \caption{Experiment results. 
    % Blue text indicates the additional results compared with the manuscript. 
    Train(s) and Infer(s) time are evaluated on a single RTX 4080 using the setting in DreamBooth. 
    % Training time is examined with batch size 4, step 500 (default setting in DreamBooth code). Inference is evaluate in 50 steps.
    }
    \vspace{-16pt}
    \label{tab:cvpr2025_rebuttal}
\end{table}


% \begin{table}[t]
%     \centering
%     \begin{adjustbox}{width=\linewidth}
% 	\begin{threeparttable}
%         \begin{tabular}{l|c|ccc|c}
%             \toprule
%             Method & Venue & CLIP-V $\uparrow$ & CLIP-V-O $\uparrow$ & LLM $\uparrow$ & Inference(s) $\downarrow$ \\
%             \midrule
%             % DreamBooth & CVPR 2023 & 0.265 & 0.293 & 78.7\% & 2.84 \\
%             % IP-adapter & Arxiv 2023 & 0.236 & 0.311 & 73.6\% & 2.28 \\
%             % Custom Diff & CVPR 2023 & 0.255 & 0.303 & 82.7\% & 2.04 \\
%             Blip-diffusion & NeurIPS 2024 & 0.264 & 0.273 & 78.0\% & 2.91 \\
%             FreeCustom & CVPR 2024 & 0.243 & 0.297 & 82.9\% & 23.78 \\
%             InstantStyle & Arxiv 2024 & 0.233 & 0.299 & 71.6\% & \textbf{1.34} \\
%             % \re{DreamMix}~\cite{yang2024dreammix} & Arxiv 2024 \\
%             \midrule
%             PhyDiff & - & \textbf{0.267} & \textbf{0.319} & \textbf{84.0\%} & 5.72 \\
%             \bottomrule
%         \end{tabular}
%         \end{threeparttable}
%     \end{adjustbox}
%     \caption{Comparison with latest methods. Inference time are evaluated on a single RTX 4080. 
%     % Training time is examined with batch size 4, step 500 (default setting in DreamBooth code). Inference is evaluate in 50 steps.
%     }
%     \vspace{-16pt}
%     \label{tab:cvpr2025_rebuttal}
% \end{table}


==> resources/tables/hyper_parameters.tex <==
%%%%%%%%%%%%% 2023/07/25 update %%%%%%%%%%%%%

\begin{table}[t]
    \centering
    \begin{adjustbox}{width=\linewidth}
	\begin{threeparttable}
        \begin{tabular}{l|ccc|ccc}
            \toprule
            Method & $\lambda_\text{decouple}$ & $\lambda_\text{isometric}$ & $\sigma$ & CLIP-V $\uparrow$ & CLIP-V-O $\uparrow$ & LLM $\uparrow$ \\
            \midrule
            % Ours & \ding{55} & \ding{55} & 0.250 & 0.310 & 77.6\% \\
            Ours & 0.1 & 1.0 & 10 \\
            Ours & 1.0 & 1.0 & 10 & \textbf{0.267} & \textbf{0.319} & \textbf{84.0\%} \\
            Ours & 10.0 & 1.0 & 10 & \\
            \midrule
            Ours & 1.0 & 0.1 & 10 & \\
            Ours & 1.0 & 1.0 & 10 & \textbf{0.267} & \textbf{0.319} & \textbf{84.0\%} \\
            Ours & 1.0 & 10.0 & 10 & \\
            \midrule
            Ours & 1.0 & 1.0 & 10 & \textbf{0.267} & \textbf{0.319} & \textbf{84.0\%} \\
            Ours & 1.0 & 1.0 & 20 & \\
            Ours & 1.0 & 1.0 & 50 & \\
            \bottomrule
        \end{tabular}
        \end{threeparttable}
    \end{adjustbox}
    \caption{\textbf{Different hyper-parameter results.}}
    \label{tab:hyper_parameters}
\end{table}


==> resources/tables/iccv2025_rebuttal.tex <==
%%%%%%%%%%%%% 2023/07/25 update %%%%%%%%%%%%%

\begin{table}[t]
    \centering
    % \vspace{-10pt}
    \begin{adjustbox}{width=\linewidth}
	\begin{threeparttable}
        \begin{tabular}{l|ccc|c}
            \toprule
            Method & CLIP-V $\uparrow$ & CLIP-V-O $\uparrow$ & LLM $\uparrow$ & Average $\uparrow$ \\
            % \midrule
            % SD-v1.5 & 0.249 & 0.292 & 0.779 & 0.440 \\
            % SD-v1.5 + IL\&DL & \textbf{0.267} & \textbf{0.319} & \textbf{0.840} & \textbf{0.475} \\
            \midrule
            SDXL-base-1.0 & 0.258 & 0.310 & 0.836 & 0.468 \\
            % SDXL-base-1.0 + IL\&DL & 0.257 & 0.314 & 0.853 &  \\
            SDXL-base-1.0 + IL\&DL & \textbf{0.275} & \textbf{0.314} & \textbf{0.853} & \textbf{0.481} \\
            \midrule
            FLUX.1-dev & 0.251 & 0.302 & 0.821 & 0.458 \\
            FLUX.1-dev + IL\&DL & \textbf{0.283} & \textbf{0.334} & \textbf{0.877} & \textbf{0.498} \\
            % \midrule
            % VAR-d30 & \\
            % VAR-d30 + IL\&DL \\
            \bottomrule
        \end{tabular}
        \end{threeparttable}
    \end{adjustbox}
    \vspace{-6pt}
    \caption{Results of isometric loss (IL) and decouple loss (DL) on diverse architectures, showing the adaptability of our method.}
    % The results highlight the adaptability of the proposed losses to different model architectures. \TODO{write long}}
    % \vspace{-20pt}
    \label{tab:iccv2025_rebuttal}
\end{table}



